MAPE-PPI: Towards Effective and Efficient Protein-Protein Interaction Prediction via Microenvironment-Aware Protein Embedding

Protein-Protein Interactions (PPIs) are fundamental in various biological processes and play a key role in life activities. The growing demand and cost of experimental PPI assays require computational methods for efficient PPI prediction. While existing methods rely heavily on protein sequence for PPI prediction, it is the protein structure that is the key to determine the interactions. To take both protein modalities into account, we define the microenvironment of an amino acid residue by its sequence and structural contexts, which describe the surrounding chemical properties and geometric features. In addition, microenvironments defined in previous work are largely based on experimentally assayed physicochemical properties, for which the "vocabulary" is usually extremely small. This makes it difficult to cover the diversity and complexity of microenvironments. In this paper, we propose Microenvironment-Aware Protein Embedding for PPI prediction (MPAE-PPI), which encodes microenvironments into chemically meaningful discrete codes via a sufficiently large microenvironment "vocabulary" (i.e., codebook). Moreover, we propose a novel pre-training strategy, namely Masked Codebook Modeling (MCM), to capture the dependencies between different microenvironments by randomly masking the codebook and reconstructing the input. With the learned microenvironment codebook, we can reuse it as an off-the-shelf tool to efficiently and effectively encode proteins of different sizes and functions for large-scale PPI prediction. Extensive experiments show that MAPE-PPI can scale to PPI prediction with millions of PPIs with superior trade-offs between effectiveness and computational efficiency than the state-of-the-art competitors.

==> table_3.tex <==
\begin{table*}[!htbp]
\begin{center}
\vspace{-1em}
\caption{Abation study on masked modeling, vector quantization, and fine-tuning on three datasets.}
\label{tab:3}
\resizebox{0.6\textwidth}{!}{

\begin{tabular}{l|cccccc|c}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{SHS27k}} & \multicolumn{2}{c}{\textbf{SHS148k}} & \multicolumn{2}{c|}{\textbf{STRING}} & \multirow{2}{*}{\textbf{Average}} \\ \cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7}
 & \textbf{DFS} & \textbf{BFS} & \textbf{DFS} & \textbf{BFS} & \textbf{DFS} & \textbf{BFS} &  \\ \midrule
 MAPE-PPI (w/ MCM) & \underline{71.98} & \underline{70.38} & \underline{79.45} & \textbf{74.76} & \underline{86.50} & \textbf{78.26} & 76.89 \\
No Masking & 70.11 & 68.60 & 78.02 & 72.93 & 84.90 & 76.99 & 75.26 {\color[rgb]{0.4, 0.71, 0.376}(-1.63 \%)} \\
w/ MLM & 70.85 & 69.25 & 78.39 & 73.89 & 85.46 & 77.20 & 75.84 {\color[rgb]{0.4, 0.71, 0.376}(-1.05 \%)} \\
w/ MEM & 70.44 & 68.28 & 77.70 & 73.06 & 84.02 & 76.39 & 74.98 {\color[rgb]{0.4, 0.71, 0.376}(-1.91 \%)} \\
w/o VQ-VAE & 68.49 & 67.31 & 76.81 & 71.19 & 83.60 & 75.89 & 73.88 {\color[rgb]{0.4, 0.71, 0.376}(-3.01 \%)} \\
Fine-tuned Encoder & \textbf{72.56} & \textbf{70.81} & \textbf{79.94} & \underline{74.60} & \textbf{87.12} & \underline{78.09} & 77.19 {\color[rgb]{0.8, 0.227, 0.141}(+0.30 \%)} \\ 
\bottomrule
\end{tabular} \vspace{-1em}

}
\end{center}
\end{table*} 

==> table_A1.tex <==
\begin{table*}[!htbp]
\begin{center}
\vspace{-1em}
\caption{The best hyperparameter choices for each dataset and partition.}
\label{tab:A1}
\vspace{0.4em}
\resizebox{0.6\textwidth}{!}{

\begin{tabular}{cc|cccccc}
\toprule
\textbf{Dataset} & \textbf{Partition} & \textbf{\ $L$\ } & \textbf{\ $F$\ } & \textbf{\ $|\mathcal{A}|$\ } & \textbf{\ $\frac{|\mathcal{M}|}{|\mathcal{A}|}$\ } & \textbf{\ $\gamma$\ } & \textbf{\ $\eta$\ } \\ \midrule
\multirow{3}{*}{SHS27k} & Random & 4 & 128 & 1,024 & 0.15 & 1.5 & 1.0 \\
 & DFS & 5 & 128 & 512 & 0.15 & 1.0 & 1.0 \\
 & BFS & 5 & 128 & 1,024 & 0.10 & 1.0 & 1.0 \\ \midrule
\multirow{3}{*}{SHS148k} & Random & 5 & 256 & 1,024 & 0.15 & 2.0 & 1.0 \\
 & DFS & 4 & 256 & 1,024 & 0.20 & 1.5 & 1.0 \\
 & BFS & 5 & 128 & 512 & 0.20 & 1.0 & 0.5 \\ \midrule
\multirow{3}{*}{STRING} & Random & 5 & 256 & 512 & 0.15 & 1.0 & 1.0 \\
 & DFS & 4 & 128 & 1,024 & 0.15 & 1.5 & 1.0 \\
 & BFS & 4 & 128 & 512 & 0.20 & 1.0 & 1.0 \\ \bottomrule
\end{tabular}

} \vspace{-1em}
\end{center}
\end{table*} 

==> table_A3.tex <==
\begin{table*}[!htbp]
\begin{center}
\vspace{-1em}
\textcolor{modify}{\caption{Hyperparametric sensitivity on the SHS148k and STRING datasets in the DFS partition.}}
\vspace{0.5em}
\label{tab:A3}
\resizebox{1.0\textwidth}{!}{

\begin{tabular}{c|cccccc}
\toprule
$|\mathcal{A}|$ & 64 & 128 & 256 & 512 & 1,024 & 2,048 \\ \midrule
\textcolor{modify}{SHS148k}             & 73.42 & 74.98 & 77.13 & \underline{79.13} & \textbf{79.45} & 78.83 \\
\textcolor{modify}{STRING}             & 83.14 & 84.53 & 85.14 & 85.40 & \textbf{86.50} & \underline{85.94} \\ \bottomrule
\end{tabular} \quad

\begin{tabular}{c|cccccc}
\toprule
$|\mathcal{M}| / |\mathcal{A}|$ & 0.05  & 0.10  & 0.15  & 0.20  & 0.25  & 0.35  \\ \midrule
\textcolor{modify}{SHS148k}        & 78.50 & 78.84 & \underline{79.18} & \textbf{79.45} & 78.13 & 76.21 \\
\textcolor{modify}{STRING}        & 85.31 & \underline{86.12} & \textbf{86.50} & 85.82 & 85.12 & 83.75 \\ \bottomrule
\end{tabular}

} \vspace{-1em}
\end{center}
\end{table*} 
